Asymptotic distribution and sparsistency for l1-penalized parametric M-estimators with applications to linear SVM and logistic regression

Since its early use in least squares regression problems, the l1-penalization framework for variable selection has been employed in conjunction with a wide range of loss functions encompassing regression, classification and survival analysis. While a well developed theory exists for the l1-penalized least squares estimates, few results concern the behavior of l1-penalized estimates for general loss functions. In this paper, we derive two results concerning penalized estimates for a wide array of penalty and loss functions. Our first result characterizes the asymptotic distribution of penalized parametric M-estimators under mild conditions on the loss and penalty functions in the classical setting (fixed-p-large-n). Our second result explicits necessary and sufficient generalized irrepresentability (GI) conditions for l1-penalized parametric M-estimates to consistently select the components of a model (sparsistency) as well as their sign (sign consistency). In general, the GI conditions depend on the Hessian of the risk function at the true value of the unknown parameter. Under Gaussian predictors, we obtain a set of conditions under which the GI conditions can be re-expressed solely in terms of the second moment of the predictors. We apply our theory to contrast l1-penalized SVM and logistic regression classifiers and find conditions under which they have the same behavior in terms of their model selection consistency (sparsistency and sign consistency). Finally, we provide simulation evidence for the theory based on these classification examples.

==> short_proofs_of_theoretical_results.tex <==
\section{Proofs of theoretical results}
\label{section:proof}

%\{Proof of results in Section \ref{section:theory}}

%We now state and prove the results in Section \ref{section:theory}.
%Before that, we prove technical Lemma \ref{result:rescaled_recentered_objective_function} which is used in the proof of Theorem \ref{result:main_result}.

%\begin{lemma}
%\label{result:rescaled_recentered_objective_function}
%Define:
%\begin{eqnarray*}
%	V_{\theta}^{(n)}(\hat{\bbP}_{n}, \lambda_{n},  u)
%	:=
%	\sum_{i=1}^{n}
%	\left[
%	L\left(Z_{i}, \theta+\frac{ u}{q_{n}}\right)
%	-
%	L\left(Z_{i}, \theta                 \right)
%	\right]
%	+
%	\lambda_{n}
%	\cdot
%	\left[
%	T\left(\theta+\frac{ u}{q_{n}}\right)
%	-
%	T\left(\theta\right)
%	\right].
%\end{eqnarray*}
%Then:
%\begin{eqnarray}
%	q_{n}\left(\hat{\theta}_{n}(\lambda_{n})-\theta\right)
%	& = & 
%	\argmin_{ u\in \bbR^{p}}\left[V_{\theta}^{(n)}(\hat{\bbP}_{n}, \lambda_{n},  u)\right].
%\end{eqnarray}
%\begin{proof}[Proof of Lemma \ref{result:rescaled_recentered_objective_function}.]
%From the definition of $\hat{\theta}_{n}(\lambda_{n})$, we know that:
%\begin{small}
%\begin{eqnarray*}
%	\hat{\theta}_{n}(\lambda_{n})
%	& = & 
%	\argmin_{t\in \Theta}
%	\left[
%	\sum_{i=1}^{n}
%	\left[
%	L\left(Z_{i}, \theta + \frac{q_{n}\left(t-\theta\right)}{q_{n}}\right)
%	\right]
%	+
%	\lambda_{n}\cdot
%	T\left(\theta + \frac{q_{n}\left(t-\theta\right)}{q_{n}}\right)
%	\right]
%	\\
%	& = & 	
%	\argmin_{t\in \Theta}
%	\left[
%	\left[
%	\hat{\bbE}_{n}\left[L\left(\bfZ, \theta + \frac{q_{n}\left(t-\theta\right)}{q_{n}}\right)\right]
%	-
%	\hat{\bbE}_{n}\left[L\left(\bfZ, \theta\right)\right]
%	\right]
%	\left[
%	\sum_{i=1}^{n}
%	\left[
%	L\left(Z_{i}, \theta + \frac{q_{n}\left(t-\theta\right)}{q_{n}}\right)
%	-
%	L\left(Z_{i}, \theta \right)
%	\right]
%	\right]
%	+
%	\lambda_{n}\cdot
%	\left[
%	T\left(\theta + \frac{q_{n}\left(t-\theta\right)}{q_{n}}\right)
%	-
%	T\left(\theta\right)
%	\right]
%	\right].
%\end{eqnarray*} 
%\end{small}
%The result follows from making a variable transformation $ u(t) = q_{n}\cdot(t-\theta)$ and letting $\hat{ u} =  u(\hat{\theta}_{n}(\lambda_{n}))$.
%\end{proof}
%\end{lemma}

\begin{proof}[Proof of Theorem \ref{result:assembling_theorem}]
The conclusion in (a) follows easily from the triangular inequality, since for each compact set $K$:
\begin{small}
\begin{eqnarray*}
\sup_{ u\in K}
\left|
V_{\theta}^{(n)}(\hat{\bbP}_{n}, \lambda_{n},  u)
-
V_{\theta}(\bfW,  u)
\right|
& \le & 
\sup_{ u\in K}
\left|
%n\cdot\left[
%\hat{\bbE}_{n}\left[ L\left(\bfZ, \theta+\frac{ u}{q_{n}}\right)\right]
%-
%\hat{\bbE}_{n} \left[L(\bfZ, \theta)\right]
%\right]
\left[
\sum_{i=1}^{n}
\left[
L\left(Z_{i}, \theta+\frac{ u}{q_{n}}\right)
-
L\left(Z_{i}, \theta\right)
\right]
\right]
-C_{\theta}(\bfW,  u)
\right|
\\
& + & 
\sup_{ u\in K}
\left|
\lambda_{n}
\cdot
\left[
T\left(\theta+\frac{ u}{q_{n}}\right)
-T(\theta)
\right]
-\lambda\cdot G_{\theta}( u)
\right|.
\end{eqnarray*}
\end{small}

To prove (b), let 
$\hat{ u}_{n} = q_{n}\cdot\left(\hat{\theta}(\lambda_{n})-\theta\right)$ and $\hat{ u} = \arg\min \left[C_{\theta}(\bfW,  u) - \lambda\cdot G_{\theta}( u)\right]$.
%For any $\delta>0$ and $\varepsilon>0$, we must be able to pick $N$ such that
%$%\begin{eqnarray*}
%	\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\right)  <  \epsilon,
%$%\end{eqnarray*} 
%for all $n>N$.
For any compact set $K_{\varepsilon}$ and each $n$, we know:
\begin{eqnarray*}
	\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\right) 
%	& = & 
%	\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\left|\vphantom{\int}\right. \hat{ u}_{n}\in K_{\varepsilon}\right) \cdot 
%	\bbP\left(\hat{ u}_{n}\in K_{\varepsilon}\right)
%	\\
%	& & + 
%	\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\left|\vphantom{\int}\right. \hat{ u}_{n}\not\in K_{\varepsilon}\right) \cdot 
%	\bbP\left(\hat{ u}_{n}\not\in K_{\varepsilon}\right).
%	\\
	& \le & 
	\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\left|\vphantom{\int}\right. \hat{ u}_{n}\in K_{\varepsilon}\right)
	+ 
	\bbP\left(\hat{ u}_{n}\not\in K_{\varepsilon}\right).
\end{eqnarray*}
Since $\hat{ u}_{n}$ is $O_{p}(1)$, there exists a compact set $K_{\varepsilon}$ such that $\lim\limits_{n\rightarrow\infty}\bbP\left(\hat{ u}_{n} \not\in K_{\varepsilon}\right) = 0$. 
Uniform convergence over compact sets ensures the second term vanishes, since $\lim_{n\rightarrow\infty}\bbP\left(\left|\hat{ u}_{n}-\hat{ u}\right|>\delta\left|\vphantom{\int}\right. \hat{ u}_{n}\in K_{\varepsilon}\right) = 0$. 
\end{proof}

\begin{proof}[Proof of Lemma \ref{result:uniform_convergence_for_loss}]
\textbf{Proof of a) pointwise convergence:}
To establish pointwise convergence, define:
\begin{eqnarray}
	\begin{array}{rcl}
		\delta_{i,n}( u) 
		& = & 
		L(Z_{i}, \theta+\frac{ u}{\sqrt{n}}) 
		- 
		L(Z_{i}, \theta)
		\\	
		D_{i} & = & \nabla_{b}L(Z_{i}, \theta)
		\\
		R_{i,n}( u) & = & \delta_{i,n}( u) - D_{i}\frac{ u}{\sqrt{n}}
		\\
		W_{n} & = & \frac{1}{\sqrt{n}}\sum_{i=1}^{n}D_{i}
		\\
		B_{n}( u) & = & \sum_{i=1}^{n}\delta_{i,n}( u).
	\end{array}
\end{eqnarray}
In terms of these definitions, we have:
\begin{eqnarray}
	B_{n}( u) 
%	& = & 
%	n\cdot\left[
%	\hat{\bbE}_{n}\left[L\left(\bfZ, \theta+\frac{ u}{\sqrt{n}}\right)\right]
%	-
%	\hat{\bbE}_{n}\left[L(\bfZ, \theta)\right]
%	\frac{1}{n}
%	\sum_{i=1}^{n}
%	\left[
%	L\left(Z_{i}, \theta+\frac{ u}{\sqrt{n}}\right)
%	-
%	L\left(Z_{i}, \theta\right)
%	\right]
%	\right]
%	\nonumber
%	\\
	& = &
	\label{equation:bn_expansion_step_1}
	W_{n}^{T} \cdot  u + \sum_{i=1}^{n}\left[R_{i,n}( u)\right].
\end{eqnarray}
Because $\theta$ is optimal, $\bbE D_{i} = 0$ and thus $\bbE\left[B_{n}( u)\right] = \sum_{i=1}^{n}\bbE\left[R_{i,n}( u)\right]$.
Add $\bbE\left[B_{n}( u)\right]$ and subtract $\sum_{i=1}^{n}\bbE\left[R_{i,n}( u)\right]$ to the right hand side of \eqref{equation:bn_expansion_step_1}:
\begin{eqnarray*}
	B_{n}( u) 
	& = & 
	\bbE\left[B_{n}( u) \right]
	+
	W_{n}^{T} u 
	+ 
	\sum_{i=1}^{n}\left[R_{i,n}( u)-\bbE\left[ R_{i,n}( u)\right]\right].
\end{eqnarray*}

Pointwise convergence for each $ u$ follows from obtaining a quadratic approximation to $\bbE\left[B_{n}( u)\right]$, a weak convergence for $W_{n}^{T} u$ and proving that the last term is $o_{p}(1)$.
These facts are established next.

\textbf{i) Quadratic approximation to $\bbE\left[B_{n}( u)\right]$:}
	First notice that 
%	this term is just the difference of the risk function evaluated at  $\theta$ and $\theta+\frac{ u}{\sqrt{n}}$:
	\begin{eqnarray*}
		\bbE\left[B_{n}( u)\right]
%		& = & 
%		n\cdot
%		\bbE\left[
%		\frac{1}{n}
%		\sum_{i=1}^{n}
%		\left[
%		L\left(Z_{i}, \theta+\frac{ u}{\sqrt{n}}\right)
%		-
%		L\left(Z_{i}, \theta\right)
%		\right]
%		\hat{\bbE}_{n}\left[L\left(\bfZ, \theta+\frac{ u}{\sqrt{n}}\right)\right]
%		-
%		\hat{\bbE}_{n}\left[L(\bfZ, \theta)\right]
%		\right]
%		\\
%		& = & 
%		n\cdot\left[
%		\bbE\left[L\left(\bfZ, \theta+\frac{ u}{\sqrt{n}}\right)\right]
%		-
%		\bbE\left[L(\bfZ, \theta)\right]		
%		\right]
%		\\
		& = & 
		n\cdot\left[
		R\left(\theta+\frac{ u}{\sqrt{n}}\right)
		-
		R\left(\theta\right)
		\right]
	\end{eqnarray*}
	
	Because the risk function $R$ is twice differentiable (L2.c) and $\theta$ is optimal, the gradient of the risk with respect to its argument $t$ must be zero at $t=\theta$.
	In addition, using the Hessian $H(\theta)$ of the risk at $\theta$, we get
	\begin{eqnarray*}
		\bbE\left[B_{n}( u)\right]
%		& = & 
		=
		n\cdot \left[\frac{ u^{T}}{\sqrt{n}}\cdot\left[H(\theta)\vphantom{\frac{ u}{\sqrt{n}}}\right]\cdot\frac{ u}{\sqrt{n}}
		+
		o\left(\left(\frac{|u|}{\sqrt{n}}\right)^{2}\right)\right]
%		\\
%		& = & 
		=
		u^{T}H(\theta) u
		+
		o(1).
	\end{eqnarray*}
	
\textbf{ii) Weak convergence of $W_{n}^{T} u$:} As above,optimality of $\theta$ implies that $\bbE\left[ D_{i} \right]= 0$ and hence $\bbE\left[W_{n}\right]=0$.
Since $\nabla_{b}L(Z, b)$ exists almost everywhere, all terms in the summation defining $W_{n}^{T}$ almost surely exist. 
Since these terms are i.i.d. and each has finite variance, the Central Limit yields
	\begin{eqnarray*}
		W_{n}\convinlaw N\left(0, J(\theta)\right), \mbox{ with } J(\theta) = \bbE\left[\nabla_{t}L(\bfZ, \theta)\nabla_{t}L(\bfZ, \theta)^{T}\right].
	\end{eqnarray*}
	
\textbf{iii) $\sum_{i=1}^{n}\left[R_{i,n}( u)-\bbE\left[ R_{i,n}( u)\right]\right]$ is $o_{p}(1)$:}
	Let $\xi_{i} = R_{i,n}( u)-\bbE\left[R_{i,n}( u)\right]$.
%	Since convergence in quadratic mean implies convergence in probability, 
	It is enough to prove that $\bbP \left|\sum_{i=1}^{n} \xi_{i}\right|^{2} = o(1)$.
	Clearly $\bbE\xi_{i} = 0$ for all $i$. 
	That, along with independence across the observed samples, yields
	\begin{eqnarray*}
		\begin{array}{rcl}
		\bbE\left[ \left|\sum_{i=1}^{n} \xi_{i}\right|^{2}\right] 
		& = &  
		\var\left[ \sum_{i=1}^{n} \xi_{i}\right] 
		=  
		\sum_{i=1}^{n}\var\left[  \xi_{i}\right]
		\\
%		& = & 
%		\sum_{i=1}^{n}\left(\bbE\left[  \left|R_{i, n}( u)\right|^{2}\right] - \left[\bbE\left(R_{i, n}( u)\right)\right]^{2}\right)
%		\\
		& \le & 
		\sum_{i=1}^{n}\left(\bbE\left[  \left|R_{i, n}( u)\right|^{2}\right]\right)
		.
		\end{array}
	\end{eqnarray*}
	Using $L(Z_{i}, t)$ almost sure differentiability at $t = \theta$, we get
%	\begin{eqnarray*}
$		\left|R_{i,n}( u)\right|^{2} 
%		& = & 
		 =  
		\left|L\left(Z_{i}, \theta+\frac{ u}{\sqrt{n}}\right)
		-
		L(\bfZ_{i}, \theta)
		-\nabla_{b}L(Z_{i}, \theta)\cdot\frac{ u}{\sqrt{n}}\right|^{2}
		= 
		o\left(\frac{1}{n}\right),		
$, for almost all $Z_{i}$.
%	\end{eqnarray*}
	It follows that $\bbE\left[\sum_{i=1}^{n} \left|R_{i, n}( u)\right|^{2}\right] = o(1)$.
	
\textbf{Proof of b.1) uniform convergence over compact sets:}

Uniform convergence of $B_{n}( u)$ over compact sets follows from the pointwise convergence just proven and the Convexity Lemma due to \citet{pollard:1991:asymptotics-for-least-absolute-deviation-regression-estimators}.

\paragraph{Proof of b.2) boundedness of $\sqrt{n}\cdot \hat{\theta}(0)$:}
	
	Our proof of $\sqrt{n}$-boundedness of the un-penalized estimate is an adaptation of an argument due to \citet{pollard:1991:asymptotics-for-least-absolute-deviation-regression-estimators}.
	As a first step, we ``complete the squares'' in the quadratic approximation by letting $C$ be a decomposition of the (non-singular) Hessian matrix, i.e. $C^{T}C = H(\theta)$. 
	We then write $B_{n}( u)$ as:
	\begin{eqnarray*}
		B_{n}( u) 
		& = & 
		\left\|C u + \frac{1}{2}(C^{-1})^{T}\bfW_{n}\right\|^{2}
		-
		\left\|\frac{1}{2}(C^{-1})^{T}\bfW_{n}\right\|^{2}
		+
		r_{n}( u),
	\end{eqnarray*}
	Let $A_{n}$ denote the ball with center $-\frac{1}{2}(C^{-1})^{T}\bfW_{n}$ and radius $\delta>0$. Since $\bfW_{n}$ converges in distribution, it is stochastically bounded and, hence, a compact set $K^{*}$ with probability arbitrarily close to one can be chosen to contain $A_{n}$. Thus:
	\begin{eqnarray*}
		\Delta_{n} & := & \sup_{ u \in A_{n}}|r_{n}( u)| \convinprob 0.
	\end{eqnarray*}
	We now study the behavior of $B_{n}$ outside of $A_{n}$ to conclude that $\hat{\theta}_{n}(0)$ is consistent.
	To do that, let $z$ be a point outside the ball and define:
	\begin{eqnarray*}
		m 
		& = & 
		\|z - \frac{1}{2}(C^{-1})^{T}\bfW_{n}\|_{2}
		\\
		v 
		& = &  
		\frac
		{z - \frac{1}{2}(C^{-1})^{T}\bfW_{n}}
		{m}
	\end{eqnarray*}
	Because of convexity, we have that for $ u^{*}=-\frac{1}{2}C^{-1}(C^{-1})^{T}\bfW_{n}+\delta \cdot v$ on the boundary of the $A_{n}$ ball:
	\begin{eqnarray*}
		\left(\frac{\delta}{m}\right)B_{n}(z)
		+
		\left(1-\frac{\delta}{m}\right)
		B_{n}\left(\frac{1}{2}(C^{-1})^{T}\bfW_{n}\right)
		& \ge &
		B_{n}( u^{*})
		\\
		& \ge & \inf\limits_{|v|\le1}\left(v^{T}H(\theta)v\right)
		-
		\frac{1}{4}\bfW_{n}^{T}\left[H(\theta)\right]^{-1}\bfW_{n}
		-
		\Delta_{n}
		\\
		& \ge & \delta^{2}\inf\limits_{|v|\le1}\left(v^{T}H(\theta)v\right)
		-
		\frac{1}{4}\bfW_{n}^{T}\left[H^{-1}(\theta)\right]\bfW_{n}
		-
		\Delta_{n}		
		\\
		& \ge & 
		\delta^{2}\Lambda_{p}(H(\theta))
		-
		B_{n}\left(-\frac{1}{2}C^{-1}(C^{-1})^{T}\bfW_{n}\right)
		-
		2\Delta_{n},		
	\end{eqnarray*}
	where $\Lambda_{p}(H(\theta))$ is the smallest eigenvalue of $H(\theta)$.
	We then conclude that:
	\begin{eqnarray*}
		\inf\limits_{\left| u+\frac{1}{2}(C^{-1})^{T}\bfW_{n}\right|>\delta}
		B_{n}( u)
		\ge
		B_{n}(-\frac{1}{2}(C^{-1})^{T}\bfW_{n})
		+
		\frac{m}{\delta}\left[\delta^{2}\Lambda_{p}(H(\theta))-2 \Delta_{n}\right].
	\end{eqnarray*}
	Since $\Delta_{n}\convinprob 0$, we have that with probability approaching one that $\left|\hat{ u}+\frac{1}{2}(C^{-1})^{T}\bfW_{n}\right|<\delta$ and the result follows from recalling that $\hat{ u} = \sqrt{n}(\hat{\theta}_{n}(0)-\theta)$.
\end{proof}


\begin{proof}[Proof of Lemma \ref{result:uniform_convergence_for_penalty}]
From the triangular inequality, we know that 

\begin{small}
\begin{eqnarray*}
	&
	\sup\limits_{ u\in K\subset \bbR^{p}}
	\left\|
	\lambda_{n}\cdot\left[T(\theta + \frac{ u}{q_{n}}) - T(\theta)\right]
	-
	\lambda\cdot G_{\theta}( u)
	\right\|
	 \le
	&
	\\ 
	&
	\sup\limits_{ u\in K\subset \bbR^{p}}
	\left\|
	\left(\frac{\lambda_{n}}{q_{n}}-\lambda\right)\cdot\left[
	\frac{T(\theta +  u\cdot q^{-1}_{n}) - T(\theta)}{q_{n}^{-1}}
	\right]
	\right\|
	+
	\sup\limits_{ u\in K\subset \bbR^{p}}
	\left\|
	\lambda\cdot
	\left(
	\frac{T(\theta +  u\cdot q^{-1}_{n}) - T(\theta)}{q_{n}^{-1}}-G_{\theta}( u)
	\right)
	\right\|,
	&
\end{eqnarray*}
\end{small}
for any compact set $K\subset \bbR^{p}$.
$T$ is continuous, so there exists $0<M_{K}<\infty$ such that
\begin{eqnarray*}
	\sup_{ u\in K\subset \bbR^{p}}
	\left\|
	\left(\frac{\lambda_{n}}{q_{n}}-\lambda\right)\cdot\left[
	\frac{T(\theta +  u\cdot q^{-1}_{n}) - T(\theta)}{q_{n}^{-1}}
	\right]
	\right\|
	& \le & 
	\left\|
	\left(\frac{\lambda_{n}}{q_{n}}-\lambda\right)
	\right\|
	\cdot M_{K}
	\convinprob 0,
\end{eqnarray*}
as $n \rightarrow \infty$.
For the second term, condition P4 in Assumption Set 2 gives
\begin{eqnarray*}
	\lim_{n\rightarrow \infty}
	\frac{T(\theta +  u\cdot q_{n}^{-1}) - T(\theta)}{q_{n}^{-1}}
	& = & 
	\lim_{h \downarrow 0}
	\frac{T(\theta + h\cdot  u) - T(\theta)}{h} = G_{\theta}( u).
\end{eqnarray*}
Because $G_{\theta}$ is assumed continuous, the pointwise convergence can be strengthened to uniform convergence over compact sets.
\end{proof}

%\subsection{Proof of results in Section \ref{section:application}}

%We now prove the results in Section \ref{section:application}.
%The main result is Theorem \ref{result:generalized_irrepresentability_condition}.
%Before we prove it, we state and prove an auxiliary lemma (Lemma \ref{result:convergence_of_l1_norm}).
%We then prove Lemmas
%\ref{result:variance_and_hessian_for_hinge_loss}, and 
%\ref{result:variance_and_hessian_for_logistic_loss}, 
%\ref{result:variance_and_hessian_for_quantile_loss} 
%which
%establish conditions for the hinge and logistic regression losses to satisfy Assumption Set 1.

%\begin{lemma}
%\label{result:convergence_of_l1_norm}
%Suppose that $\frac{\lambda_{n}}{n^{\frac{1}{2}-c}} \rightarrow \lambda$ as $n\rightarrow\infty$.
%Then, as $n\rightarrow\infty$:
%\begin{eqnarray*}
%	\sup_{ u\in K}
%	\left|
%	\lambda_{n} 
%	\cdot 
%	n^{c}
%	\cdot
%	\left[
%	\left\|\beta+\frac{ u}{\sqrt{n}}\right\|_{1}-\left\|\beta\right\|_{1}
%	\right]
%	- 
%	\lambda 
%	\cdot
%	\left[
%	\left(\sum_{j: \beta_{j}=0}\left|u_{j}\right|\right) + \left(\sum_{j:\beta_{j}\neq 0}u_{j}\cdot\sign(\beta_{j})\right)
%	\right]
%	\right|
%	\rightarrow 
%	0, 
%\end{eqnarray*}
%for all compact subsets $K\subset \bbR^{p}$.
%\end{lemma}

%\begin{proof}[Proof of Lemma \ref{result:convergence_of_l1_norm}]
%Lemma \ref{result:convergence_of_l1_norm} has been previously proved by \citet{knight:2000:asymptotics} and we include it here for completeness.
%The proof of Lemma \ref{result:convergence_of_l1_norm} can be easily established by noticing that the $\ell_{1}$-norm penalty satisfies all conditions in Lemma \ref{result:uniform_convergence_for_penalty} and:
%\begin{eqnarray*}
%	\lambda_{n}\cdot n^{c}\cdot\left(\left\|\beta+\frac{ u}{\sqrt{n}}\right\|_{1}-\left\|\beta\right\|_{1}\right)
%	& = &
%	\frac{\lambda_{n}}{n^{\frac{1}{2}-c}}
%	\cdot
%	\left[
%	\sum_{j:\beta_{j}=0}\left| u_{j}\right|
%	+
%	\sum_{j:\beta_{j}>0}\left(\left|\sqrt{n}\cdot\beta_{j}+ u_{j}\right|_{1}-\sqrt{n}\cdot\beta_{j}\right)
%	\right]
%	\\
%	&&
%	+
%	\frac{\lambda_{n}}{n^{\frac{1}{2}-c}}
%	\cdot
%	\left[
%	\sum_{j:\beta_{j}<0}\left(\left|\sqrt{n}\cdot\beta_{j}+ u_{j}\right|_{1}+\sqrt{n}\cdot\beta_{j}\right)
%	\right]
%	\\
%	& = & 
%	\frac{\lambda_{n}}{n^{\frac{1}{2}-c}}
%	\left[
%	\left(\sum_{j: \beta_{j}=0}\left|u_{j}\right|\right) + \left(\sum_{j:\beta_{j}\neq 0}u_{j}\cdot\sign(\beta_{j})\right)
%	\right],
%\end{eqnarray*}
%for large enough $n$.
%\end{proof}

\begin{proof}[Proof of Theorem \ref{result:generalized_irrepresentability_condition}]
For the $\ell_{1}$-penalty, the difference between 
%\begin{eqnarray*}
$	\lambda_{n}\left(\|\beta+\frac{u}{\sqrt{n}}\|_{1}-\|\beta\|_{1}\right)
    -
	\frac{\lambda_{n}}{\sqrt{n}}\left(u_{\mcalA}-\|u_{\mcalA^{c}}\|_{1}\right)
	\rightarrow
	0,$
%\end{eqnarray*}	
uniformly as $n\rightarrow \infty$.
Using Theorem \ref{result:assembling_theorem} and Lemma \ref{result:uniform_convergence_for_loss},
\begin{eqnarray*}
%	\label{equation:limit_distribution_l1_penalized_estimates}
	\sqrt{n}\left(\hat{\theta}_{n}(\lambda_{n})-\theta\right)
	\convinlaw 
	\hat{ u}
	:=
	\argmin_{ u} 
	\left[
	 u^{T} H(\theta) u + \bfW^{T} u + 
	\frac{\lambda_{n}}{\sqrt{n}}\left(u_{\mcalA} + \left\| u_{\mcalA^{c}}\right\|_{1}\right)
	\right],
\end{eqnarray*}
with $\bfW\sim N\left(0, J(\theta)\right)$.
%The proof then follows similar steps as \citet{zhao:2006:lasso_model_selection_consistency} which we detail below.
%
%The random vectors $\hat{ u}_{\mcalA}$ and $\hat{ u}_{\mcalA^{c}}$ for the penalized indices determine the correctness of the signs of $\hat{\beta}(\lambda_{n})$ in the limit.
We assume, without loss of generality that $\beta_{\mcalA}>0$ with the inequality holding element-wise.
In that case:
\begin{eqnarray*}
	\begin{array}{lllll}
		\sign(\hat{\beta}_{j}(\lambda_{n})) = \sign(\beta_{j}) 
		& \Leftrightarrow & 
		\frac{\hat{ u}_{j}}{\sqrt{n}} \ge -\beta_{j}, 
		&
		\mbox{ for } j\in \mcalA,
		\\
		\sign(\hat{\beta}_{j}(\lambda_{n})) = \sign(\beta_{j}) 
		& \Leftrightarrow & 
		\hat{ u}_{j} = 0, 
		&
		\mbox{ for } j\in \mcalA^{c}.
	\end{array}
\end{eqnarray*}
%
For the remainder of this proof, we drop denote $H(\theta)$ by $H$.
In terms of the $\alpha$, $\mcalA$, $\mcalA^{c}$ partition, the Karush-Kuhn-Tucker (KKT) conditions for optimization defining $\hat{u}$ above are
\begin{eqnarray*}
	\begin{array}{rllll}
		H_{\alpha    , \mcalA    }\cdot\hat{ u}_{\mcalA}
		+
		H_{\alpha    , \mcalA^{c}}\cdot\hat{ u}_{\mcalA^{c}}
		+
		H_{\alpha    , \alpha    }\cdot\hat{ u}_{\alpha}
		+
		\bfW_{\alpha   }
		& = & 
		0,
		\\
		H_{\mcalA    , \mcalA    }\cdot\hat{ u}_{\mcalA}
		+
		H_{\mcalA    , \mcalA^{c}}\cdot\hat{ u}_{\mcalA^{c}}
		+
		H_{\mcalA    , \alpha    }\cdot\hat{ u}_{\alpha}
		+
		\bfW_{\mcalA   }
		-
		\frac{\lambda_{n}}{\sqrt{n}}
		& = & 
		0,
		\\
		H_{j         , \mcalA    }\cdot\hat{ u}_{\mcalA}
		+
		H_{j         , \mcalA^{c}}\cdot\hat{ u}_{\mcalA^{c}}
		+
		H_{j         , \alpha    }\cdot\hat{ u}_{\alpha}
		+
		\bfW_{j}
		-
		\frac{\lambda_{n}}{\sqrt{n}}\cdot
		\sign(\hat{ u}_{j})
		& = & 
		0,
		\\
		\mbox{ for } j \in \mcalA^{c} \mbox{ s.t. } \hat{u}_{j}\neq 0  
		&
		& 
		\\
		\left|
		H_{j         , \mcalA    }\cdot\hat{ u}_{\mcalA    }
		+
		H_{j         , \mcalA^{c}}\cdot\hat{ u}_{\mcalA^{c}}
		+
		H_{j         , \alpha    }\cdot\hat{ u}_{\alpha}
		+
		\bfW_{j}
		\right|
		& \le & 
		\frac{\lambda_{n}}{\sqrt{n}},
		\\
		\mbox{ for } j \in \mcalA^{c} \mbox{ s.t. } \hat{u}_{j}= 0  
		& 
		&
	\end{array}
\end{eqnarray*}
To select the zero terms in $\beta$ correctly, we must have $\hat{ u}_{\mcalA^{c}=0}$. 
In that case,
\begin{eqnarray*}
	\left[
	\begin{array}{c}
	\hat{ u}_{\alpha}
	\\
	\hat{ u}_{\mcalA}		
	\end{array}
	\right]
	& = & 
	\left[
	\begin{array}{cc}
	H_{\alpha, \alpha} & H_{\mcalA, \alpha}
	\\
	H_{\mcalA, \alpha} & H_{\mcalA, \mcalA}
	\end{array}
	\right]^{-1}
	\cdot
	\left[
	\begin{array}{c}
	\bfW_{\alpha}
	\\
	\frac{\lambda_{n}}{n}\cdot\bfone_{q} - \bfW_{\mcalA}
	\end{array}
	\right].
%	\\
%	& = & 
%	\left[
%	\begin{array}{c}
%	\left[H_{\alpha, \alpha}-H_{\alpha, \mcalA}H_{\mcalA, \mcalA}^{-1}H_{\mcalA, \alpha}\right]^{-1}
%	\cdot
%	\left[\bfW_{\alpha}	
%	-
%	\left[H_{\alpha, \mcalA}H_{\mcalA, \mcalA}^{-1}\right]\cdot \left(\frac{\lambda_{n}}{\sqrt{n}} - \bfW_{\mcalA}\right)
%	\right]
%	\\
%	\left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}
%	\cdot 
%	\left[ 
%	\left(\frac{\lambda_{n}}{\sqrt{n}}\cdot\bfone_{q} - \bfW_{\mcalA}\right)
%	-
%	\left[H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}\right]\cdot \bfW_{\alpha}
%	\right]
%	\end{array}
%	\right].
\end{eqnarray*}
Define a zero mean Gaussian random vector $\tilde{\bfW} = \left[\begin{array}{cc}\tilde{\bfW}_{\mcalA}, & \tilde{\bfW}_{\mcalA^{c}}\end{array}\right]$ :
\begin{small}
\begin{eqnarray*}
	\tilde{\bfW}_{\mcalA}     & := & 
	-
	\mcalH
	\cdot
	\left[\bfW_{\mcalA} + H_{\mcalA, \alpha}\cdot H_{\alpha, \alpha}^{-1} \cdot \bfW_{\alpha}\right], \mbox{ and }
	\\
	\tilde{\bfW}_{\mcalA^{c}} & := & 
	\bfW_{\mcalA^{c}} 
	-
	\left[
	\begin{array}{c}
	H_{\mcalA^{c}, \alpha}
	\\
	H_{\mcalA^{c}, \mcalA}
	\end{array}
	\right]
	^{T}
	\left[
	\begin{array}{cc}
	H_{\alpha, \alpha}	&	H_{\alpha, \mcalA}\\
	H_{\mcalA, \alpha}	&	H_{\mcalA, \mcalA}
	\end{array}
	\right]
	^{-1}
	\left[
	\begin{array}{c}
	\bfW_{\alpha}
	\\
	\bfW_{\mcalA}
	\end{array}
	\right], \mbox{ with }\\
	\mcalH & := & \left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}
\end{eqnarray*}
\end{small}
%Using Schur's inversion formula for partitioned matrices, we get:
%\begin{eqnarray*}
%	\hat{ u}_{\mcalA}
%	& = & 
%	\left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}
%	\cdot 
%	\left[ 
%	\frac{\lambda_{n}}{\sqrt{n}}\cdot\bfone_{q} 
%	- 
%	\bfW_{\mcalA}
%	-
%	\left[H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}\right]\cdot \bfW_{\alpha}
%	\right].
%\end{eqnarray*}
%
%For the signs of all estimates to agree, we must have:
%\begin{small}
%\begin{eqnarray*}
%	-
%	\left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}
%	\cdot 
%	\left[ 
%	\frac{\lambda_{n}}{\sqrt{n}}\cdot\bfone_{q} 
%	- 
%	\bfW_{\mcalA}
%	-
%	\left[H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}\right]\cdot \bfW_{\alpha}
%	\right]
%	&
%	<
%	&  
%	\sqrt{n}\cdot\beta_{\mcalA},
%	\mbox{ and }
%	\\
%	\left\|
%	\bfW_{\mcalA^{c}} 
%	-
%	\left[
%	\begin{array}{c}
%	H_{\mcalA^{c}, \alpha}
%	\\
%	H_{\mcalA^{c}, \mcalA}
%	\end{array}
%	\right]
%	^{T}
%	\left[
%	\begin{array}{cc}
%	H_{\alpha, \alpha}	&	H_{\alpha, \mcalA}\\
%	H_{\mcalA, \alpha}	&	H_{\mcalA, \mcalA}
%	\end{array}
%	\right]
%	^{-1}
%	\left[
%	\begin{array}{c}
%	\bfW_{\alpha}
%	\\
%	\bfW_{\mcalA}
%	\end{array}
%	\right]
%	\right\|_{\infty}
%	& \le & 
%	\frac{\lambda_{n}}{\sqrt{n}}
%	\left(
%	1
%	-
%	H_{\mcalA^{c}, \mcalA}
%	\left[H_{\mcalA, \mcalA}\right]^{-1}
%	\right).
%	\mbox{ and }
%	\\
%	\frac{\lambda_{n}}{\sqrt{n}}
%	\left(
%	1
%	-
%	H_{\mcalA^{c}, \mcalA}
%	\left[H_{\mcalA, \mcalA}\right]^{-1}
%	\right)
%	& \ge &  
%	\bfW_{\mcalA^{c}} 
%	-
%	\left[
%	\begin{array}{c}
%	H_{\mcalA^{c}, \alpha}
%	\\
%	H_{\mcalA^{c}, \mcalA}
%	\end{array}
%	\right]
%	^{T}
%	\left[
%	\begin{array}{cc}
%	H_{\alpha, \alpha}	&	H_{\alpha, \mcalA}\\
%	H_{\mcalA, \alpha}	&	H_{\mcalA, \mcalA}
%	\end{array}
%	\right]
%	^{-1}
%	\left[
%	\begin{array}{c}
%	\bfW_{\alpha}
%	\\
%	\bfW_{\mcalA}
%	\end{array}
%	\right].
%\end{eqnarray*}
%\end{small}
The M-estimated parameter fails to have the correct signs if either:
\begin{small}
\begin{eqnarray*}
	\begin{array}{lllll}
	\tilde{\bfW}_{j}	
	& \ge &
	\sqrt{n}\cdot \beta_{j}
	-
	\frac{\lambda_{n}}{\sqrt{n}}
	\cdot
	%\sum_{k\in \mcalA}\left[\left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}\right]_{jk},
	\sum_{k\in \mcalA}\mcalH_{jk},
	& 
	\mbox{ for some $j\in \mcalA$, } & \mbox{ OR, }
	\\
	\left|\tilde{\bfW}_{j}\right|
	& > & 
	\frac{\lambda_{n}}{\sqrt{n}}
	\left(
	1
	-
	H_{j,\mcalA}(\theta)\cdot
	\left[H_{\mcalA, \mcalA}(\theta)\right]^{-1}
	\right),
	&
	\mbox{ for some $j\in \mcalA^{c}$.}
	\end{array}
\end{eqnarray*}
\end{small}

To finish the proof, let $\Phi$ denote the standard normal cumulative distribution function, and define $\varsigma_{j}^{2}:=\var(\tilde{\bfW}_{j})$.
% and $\eta_{j}=\sum_{k\in \mcalA}\left[\left[H_{\mcalA, \mcalA}-H_{\mcalA, \alpha}H_{\alpha, \alpha}^{-1}H_{\alpha, \mcalA}\right]^{-1}\right]_{jk}$.
%For the conditions on $\tilde{\bfW}_{\mcalA}$, we get:
Then use the union bound and the inequality $1-\Phi(r)\le\exp\left[-\frac{r^{2}}{2}\right]$ for large enough $r$, to get
\begin{small}
\begin{eqnarray*}
	\bbP\left(
	\exists j\in \mcalA:
	\tilde{\bfW}_{j}
	> 
	\sqrt{n}\cdot\left(\beta_{j} - \frac{\lambda_{n}}{n}\right)
%	\mbox{ for some } j\in\mcalA
	\right)
	& \le &
%	\sum_{j\in \mcalA} 
%	\bbP\left(
%	\tilde{\bfW}_{j}
%	> 
%	\sqrt{n}\left(\beta_{j} - \frac{\lambda_{n}}{n}\right)
%	\right)	 
%	\\
%	& \le &
%	\sum_{j\in \mcalA} 
%	\bbP\left(
%	\frac{\tilde{\bfW}_{j}}{\varsigma_{j}}
%	> 
%	\sqrt{n}\left(\frac{\beta_{j}}{\varsigma_{j}} - \frac{\lambda_{n}}{n\cdot \varsigma_{j}}\right)
%	\right)	 
%	\\
%	& \le & 
%	q
%	\cdot
%	\left[1
%	-
%	\Phi\left(
%	\sqrt{n}\cdot \left(\min\limits_{j\in\mcalA}\left(\frac{\beta_{j}}{\varsigma_{j}}\right) - \frac{\lambda_{n}}{n\cdot\max\limits_{j\in\mcalA}{\varsigma_{j}}}\right)
%	\right)
%	\right]
%	\\
%	& \le &
	q\cdot
	\frac{
	\exp\left[
	-\frac{n}{2}
	\cdot 
%	\left(
%	\min\limits_{j\in\mcalA}\left(\frac{\beta_{j}}{\varsigma_{j}}\right) - \frac{\lambda_{n}^{2}}{n^{2}\cdot\max\limits_{j\in\mcalA}{\varsigma_{j}^}}
%	\right)^{2}
	s^{2}
	\right]
	}
	{
	s
	\sqrt{n}
	%\cdot\left(\min\limits_{j\in\mcalA}\left(\frac{\beta_{j}}{\varsigma_{j}}\right) - \frac{\lambda_{n}}{n\cdot\max\limits_{j\in\mcalA}{\varsigma_{j}}}\right)
	}, \mbox{ and }
%\end{eqnarray*}
%\end{small}
%Similarly, for the conditions on $\tilde{\bfW}_{\mcalA^{c}}$, we get:
%\begin{small}
%\begin{eqnarray*}	
	\\
	\bbP\left(
	\exists j\in \mcalA^{c}:
	\left|\tilde\bfW_{j}\right|
	> 
	\frac{\lambda_{n}\left(1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\right)}{\sqrt{n}}
	\right)
%	& \le &  
%	2
%	\sum_{j\in \mcalA^{c}}
%	\left[
%	1-
%	\Phi
%	\left(
%	\frac{\lambda_{n}}{\varsigma_{j}\sqrt{n}}\cdot\left(1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\right)
%	\right)
%	\right]
%	\\
	& \le &
	\frac{
	2
	(p-q)
	\exp
	\left[
	-
	\frac{\left(\lambda_{n}/\sqrt{n}\right)^{2}}{2\max\limits_{j\in \mcalA^{c}}\left(\varsigma^{2}_{j}\right)}
	\cdot
	%\left(\min\limits_{j\in\mcalA^{c}}\left(1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\right)\right)^{2}
	\eta^{2}
	\right]
	}
	{
	\frac{\lambda_{n}}{\sqrt{n}\max\limits_{j\in \mcalA^{c}}\left(\varsigma_{j}\right)}
	\cdot
	\eta
	%\min\limits_{j\in\mcalA^{c}}\left(1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\right),
	}
\end{eqnarray*}
\end{small}
with $s = \min\limits_{j\in\mcalA}\left(\frac{\beta_{j}}{\varsigma_{j}}\right) - \frac{\lambda_{n}}{n\cdot\max\limits_{j\in\mcalA}{\varsigma_{j}}}$ and $\eta = 1-\max_{j\in \mcalA^{c}}\left[H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\sign(\beta_{\mcalA})\right]$.
Since $\eta>0$, the result follows from making use of the assumptions that $\frac{\lambda_{n}}{n}\rightarrow0$ and $\frac{\lambda_{n}}{n^{\frac{1+c}{2}}}\rightarrow\infty$ as $n\rightarrow\infty$.

To prove the converse, notice that if there exists $j\in \mcalA^{c}$ with $1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\le0$, then $\bbP\left(\left|\tilde\bfW_{j}\right|> \frac{\lambda_{n}\left(1-H_{j,\mcalA}H_{\mcalA, \mcalA}^{-1}\right)}{\sqrt{n}}\right)$ is always greater than zero. Thus, there is always a non-zero chance of incorrectly picking an irrelevant variable.
\end{proof}

\begin{proof}[Proof of Theorem \ref{result:simplified_gi_condition}]
Throughout this proof we denote $\nu:=\frac{\beta}{\|\beta\|}\in \bbR^{p}$, the unit vector in the direction of $\beta$.
Using the properties of Gaussian distributions and the condition $\nu^{T}\mu=0$, we get
\begin{small}
\begin{eqnarray*}
	\begin{array}{rcl}
	\bbE\left[\bfX\bfX^{T}\left|\alpha+\bfX^{T}\beta\right.\right]
	& = &
	\mu\mu^{T}
	+
	\Sigma
	+
	\frac{\Sigma\nu\nu^{T}\Sigma}{(\nu^{T}\Sigma\nu)^{2}}
	\cdot
	\left[
	\left(
	\frac
	{\left(\alpha+\bfX^{T}\beta\right)-\left(\alpha+\beta^{T}\mu\right)}
	{\|\beta\|}
	\right)^{2}-1
	\right]
	.
	\end{array}
\end{eqnarray*}
\end{small}
%For details, we refer the reader to Appendix \ref{section:conditional_moments_of_gaussian_distributions}.
Let $f_{\bfM}$ denote the density of the random variable $\bfM=\alpha+\bfX^{T}\beta$ and define
\begin{eqnarray*}
	\kappa 
	& := &
	\int
	\left[
	\left(
	\frac
	{m-\left(\alpha+\beta^{T}\mu\right)}
	{\|\beta\|}
	\right)^{2}-1
	\right]
	\cdot 
	w(m)
	\cdot 
	\tilde{f}_{\bfM}(m)
	\cdot 
	\mbox{d}m.
\end{eqnarray*}
the Hessian of the risk function becomes:
\begin{eqnarray*}
	H(\theta)
	& = &
	\mu\mu^{T}
	+
	\Sigma 
	+
	\kappa
	\cdot
	\frac{\Sigma \nu\nu^{T} \Sigma}{\left(\nu^{T}\Sigma\nu\right)^{2}}.
\end{eqnarray*}
Partition $\nu$, $\mu$, and $\Sigma$ according to the sparsity pattern in $\nu$:
\begin{eqnarray*}
\begin{array}{ccccccccccc}
	\nu & = & \left[\begin{array}{c}\nu_{\mcalA} \\ \bfzero\end{array}\right],
	&
	\mu & = & \left[\begin{array}{c}\mu_{\mcalA} \\ \mu_{\mcalA^{c}}\end{array}\right], \mbox{ and }
	&
	\Sigma 
	& = & 
	\left[
	\begin{array}{cc}
		\Sigma_{\mcalA    ,\mcalA    } & \Sigma_{\mcalA    ,\mcalA^{c}} \\
		\Sigma_{\mcalA^{c},\mcalA    } & \Sigma_{\mcalA^{c},\mcalA^{c}} \\
	\end{array}
	\right].
\end{array}
\end{eqnarray*}
Defining $\bfA := \left(\bfI_{q}+\kappa\cdot\nu_{\mcalA}\nu_{\mcalA}^{T}\cdot\Sigma_{\mcalA, \mcalA}\right)$, the partitioned Hessian is
\begin{small}
\begin{eqnarray*}
	H(\theta)
	& = & 
	\left[
	\begin{array}{cc}
	\left(\mu_{\mcalA}\mu_{\mcalA}^{T} + \Sigma_{\mcalA    , \mcalA    }\right)
	\cdot
	%\left(\bfI_{q}+\kappa\cdot\nu_{\mcalA}\nu_{\mcalA}^{T}\cdot\Sigma_{\mcalA, \mcalA}\right)
	\bfA
	&
	\left(\bfI_{q}+\kappa\cdot\Sigma_{\mcalA, \mcalA}\cdot\nu_{\mcalA}\nu_{\mcalA}^{T}\right)
	\cdot
	%\left(\mu_{\mcalA}\mu_{\mcalA^{c}}^{T} + \Sigma_{\mcalA    , \mcalA^{c}}\right)
	\bfA
	\\
	%\left(\mu_{\mcalA^{c}}\mu_{\mcalA}^{T} + \Sigma_{\mcalA^{c}, \mcalA    }\right)
	\bfA
	\cdot
	\left(\bfI_{q}+\kappa\cdot\nu_{\mcalA}\nu_{\mcalA}^{T}\cdot\Sigma_{\mcalA, \mcalA}\right)
	&
	\mu_{\mcalA^{c}}\mu_{\mcalA^{c}}^{T}
	+
	\Sigma_{\mcalA^{c}, \mcalA^{c}} 
	+
	\kappa
	\cdot
	\Sigma_{\mcalA^{c}, \mcalA}\cdot\nu_{\mcalA}\nu_{\mcalA}^{T}\cdot\Sigma_{\mcalA    , \mcalA^{c}}
	\end{array}
	\right].
\end{eqnarray*}
\end{small}
\begin{small}
\begin{eqnarray*}
	H_{\mcalA^{c}, \mcalA}(\theta)\left[H_{\mcalA, \mcalA}(\theta)\right]^{-1}
	& = &
	\left(\mu_{\mcalA^{c}}\mu_{\mcalA}^{T} + \Sigma_{\mcalA^{c}, \mcalA    }\right)
	\cdot
	\bfA
	\times
	\left[
	\left(\mu_{\mcalA}\mu_{\mcalA}^{T} + \Sigma_{\mcalA    , \mcalA    }\right)
	\cdot
	\bfA
	\right]^{-1}
	\\
	& = &
	\left(\mu_{\mcalA^{c}}\mu_{\mcalA}^{T} + \Sigma_{\mcalA^{c}, \mcalA    }\right)
	\bfA\bfA^{-1}
	\left(\mu_{\mcalA}\mu_{\mcalA}^{T} + \Sigma_{\mcalA    , \mcalA    }\right)^{-1}
	\\
	& = &
	\left[\bbE\left(\bfX_{\mcalA^{c}, \mcalA    }\right)\right]
	\left[\bbE\left(\bfX_{\mcalA    , \mcalA    }\right)\right]^{-1}.
\end{eqnarray*}
\end{small}
The result follows from post-multiplying both sides of this last equation by $\sign(\beta_{\mcalA})$.
\end{proof}




\begin{proof}[Proof of Lemma \ref{result:variance_and_hessian_for_logistic_loss}]
%Throughout the proof of Lemma \ref{result:variance_and_hessian_for_logistic_loss}, we define $\tilde{\bfX} = \left[\begin{array}{cc}1 & \bfX^{T}\end{array}\right]^{T}$.
In the interest of space, we only outline the proof here.
A detailed proof is given in a technical report version of this paper.
Throughout the proof of Lemma \ref{result:variance_and_hessian_for_logistic_loss}, we denote $\tilde{\bfX} = \left[\begin{array}{cc}1 & \bfX^{T}\end{array}\right]^{T}$.
\\
%\begin{enumerate}
%	\item [L1)] 
\textbf{Proof of L1)}
	For the logistic regression loss function, we can prove that
	\begin{eqnarray*}
		\lim_{\|t\|_{2}\rightarrow\infty}
		\bbE\left[-\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t + \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right]
		& = &
		\infty,
	\end{eqnarray*}
	which ensures existence of a minimized. 
	Uniqueness follows from positive definiteness of the Hessian at the minimizer proven below.
%	We first prove the existence of a minimizer.
%	Given that the risk function is continuous, it is enough to prove that the closed set $\mcalS(\bfM) = \left\{t\in \bbR^{p}: \bbE\left[-\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t + \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right]\le \bfM\right\}$ for large enough $\bfM$ is bounded.
%	We establish boundedness of $\mcalS(\bfM)$ by proving that $\mcalS(\bfM)$ is contained on a finite sphere around the origin which can be established by proving  that, for any $\bfM$ there exists $\gamma$ such that:
%	\begin{eqnarray}
%		\label{equation:logistic_out_of_box_inclusion}
%		\left|\langle t, t\rangle\right| > \gamma 
%		& \Rightarrow & 
%		\bbE\left[-\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t + \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right]>\bfM.
%	\end{eqnarray}
%	To prove the assertion in \eqref{equation:logistic_out_of_box_inclusion}, let $t$ be a non-zero vector with $u = \sqrt{\langle t, t\rangle} \neq 0$, so $t$ can be written as $t = u v$, for some $v\neq 0$. For any $u_{0}\in \bbR$, we can write:
%	\begin{small}
%	\begin{eqnarray*}
%		\begin{array}{ccc}
%		\bbE\left[-u\cdot\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}v + \log\left(1+\exp\left(u\cdot \tilde{\bfX}^{T}v\right)\right)\right]
%		& = & 
%		\\
%		-u\cdot\bbE\left[p(\bfX)\cdot \tilde{\bfX}^{T}v\right]
%		+ 
%		\bbE\left[\log\left(1+\exp\left(u \cdot\tilde{\bfX}^{T}v\right)\right)\right]
%		& \ge & 
%		\\
%		-u\cdot\bbE\left[p(\bfX)\cdot \tilde{\bfX}^{T}v\right]
%		+ 
%		\bbE\left[\log\left(1+\exp\left(u_{0} \cdot\tilde{\bfX}^{T}v\right)\right)\right]
%		+ 
%		\bbE
%		\left[
%		\frac
%		{\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		{1+\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right]
%		\cdot
%		(u-u_{0})
%		& = & 
%		\\
%		c(u_{0}, v)
%		+
%		\bbE\left[
%		\left(
%		\frac
%		{\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		{1+\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		-
%		p(\bfX)
%		\right)
%		\cdot 
%		\tilde{\bfX}^{T}v\right]
%		\cdot
%		u,
%		\end{array}
%		\\
%		-u\cdot\bbE\left[p(\bfX)\cdot \tilde{\bfX}^{T}v \right] 
%		+ 
%		\log\left(1+\exp\left(u \cdot\bbE\left(\tilde{\bfX}^{T}v\right)\right)\right)
%		& \ge & 
%		\\
%		-u\cdot\bbE\left[p(\bfX)\cdot \tilde{\bfX}^{T}v \right] 
%		+ 
%		\log\left(1+\exp\left(u_{0}\cdot\bbE\left(\tilde{\bfX}^{T}v\right)\right)\right)
%		+
%		\frac
%		{\exp\left(u_{0}\cdot \bbE\left(\tilde{\bfX}^{T}v\right)\right)}
%		{1+\exp\left(u_{0}\cdot \bbE\left(\tilde{\bfX}^{T}v\right)\right)}
%		\cdot 
%		\bbE\left(\tilde{\bfX}^{T}v\right)
%		\cdot 
%		u
%		-
%		\frac
%		{\exp\left(u_{0}\cdot \bbE\left(\tilde{\bfX}^{T}v\right)\right)}
%		{1+\exp\left(u_{0}\cdot \bbE\left(\tilde{\bfX}^{T}v\right)\right)}
%		\cdot 
%		\bbE\left(\tilde{\bfX}^{T}v\right)
%		\cdot 
%		u_{0}.
%	\end{eqnarray*}
%	\end{small}
%	where the inequality follows from convexity of the mapping $s\mapsto \log\left(1+\exp\left(s \cdot\tilde{\bfX}^{T}v\right)\right)$ and $c(u_{0}, v) = 
%		\bbE\left[\log\left(1+\exp\left(u_{0} \cdot\tilde{\bfX}^{T}v\right)\right)\right]
%		-	
%		\bbE
%		\left[
%		\frac
%		{\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		{1+\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right]
%		\cdot
%		u_{0}$, which does not involve $u$.
%	
%	Under the assumptions made, we can use the dominated convergence theorem to get:
%	\begin{eqnarray*}
%		\lim_{u_{0}\rightarrow\infty}
%		\bbE
%		\left[
%		\left(
%		\frac
%		{\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		{1+\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		-
%		p(\bfX)
%		\right)
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right]
%		& = & 
%		\bbE
%		\left[
%		\left(
%		1		
%		-
%		p(\bfX)
%		\right)
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right], \mbox{ and }
%		\\
%		\lim_{u_{0}\rightarrow-\infty}
%		\bbE
%		\left[
%		\left(
%		\frac
%		{\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		{1+\exp\left(u_{0}\cdot \tilde{\bfX}^{T}v\right)}
%		-
%		p(\bfX)
%		\right)
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right]
%		& = & 
%		-
%		\bbE
%		\left[
%		p(\bfX)
%		\cdot 
%		\tilde{\bfX}^{T}v
%		\right].
%	\end{eqnarray*}
%	Since the density is everywhere positive, the hyperplane $\{\bfs\in \bbR^{p+1}:\bfs^{T}v=0\}$ has probability zero for any $v\neq0$ and thus we have either $\bbE\left(\tilde{\bfX}v\right)>0$ or $\bbE\left(\tilde{\bfX}v\right)<0$.
%
%	If $\bbE\left(\tilde{\bfX}v\right)>0$, pick $u_{0}$ large enough so $\bbE\left[\left(1-p(\bfX)\right)\cdot \tilde{\bfX}^{T}v \right]>0$ to conclude that 			
%	\begin{eqnarray*}
%		\lim_{u\rightarrow\infty}\bbE\left[-\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t + \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right]=\infty.
%	\end{eqnarray*}
%
%	If, on the other hand, $\bbE\left(\tilde{\bfX}v\right)<0$, pick $u_{0}$ small enough so $\bbE\left[p(\bfX)\cdot \tilde{\bfX}^{T}v \right]<0$ to conclude:
%	\begin{eqnarray*}
%		\lim_{u\rightarrow\infty}\bbE\left[-\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t + \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right]=\infty.
%	\end{eqnarray*}
%
%	This establishes that for any $\bfM$ there exists $\gamma$ such that the risk function exceeds $\bfM$ and completes the proof of existence.
%	
%	The proof of uniqueness follows from strict convexity of the risk function.
%	We prove that below by showing that the Hessian matrix of the risk function is everywhere strictly positive definite under the assumptions made.
	
\textbf{Proof of L2)}
%	\item [L2)]	
	For the canonical logistic regression loss function, we have:
	\begin{eqnarray*}
		\bbE\left[\left|L(\bfY, \bfX, t)\right|\right]
		%& = & 
		%\bbE\left[\left|\bbI(\bfY=1)\cdot \tilde{\bfX}^{T}t - \log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right|\right]
		%\\
		& \le & 
		%\bbE\left[\left|\tilde{\bfX}\right|\right]^{T}t
		%+
		%\bbE\left[\left|\log\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)\right|\right]
		%\\
		%& = & 
		\bbE\left[\left|\tilde{\bfX}\right|\right]^{T}t
		+
		\log\left(2\right)+2\cdot\bbE\left[|\tilde{\bfX}^{T}t|\right].
	\end{eqnarray*}
	%where the equality follows from $\exp(\tilde{\bfX}^{T}t)\ge0$ for all $t$.
	The result follows from $\bbE\left|\bfX\right|$ being bounded.

\textbf{Proof of L3)}
%	\item [L3)]
	The canonical logistic regression loss function is twice differentiable everywhere, with
	%\begin{eqnarray*}
		$\nabla_{t}L(\bfY, \bfX, t) 
	%	& = &
		=
		\left[\bbI\left(\bfY=1\right) - \frac{\exp\left(\tilde{\bfX}^{T}t\right)}{1+\exp\left(\tilde{\bfX}^{T}t\right)}\right]\cdot\tilde{\bfX}$, 
	%	\mbox{ and }
		and
	%	\\
		$
		\nabla_{t}^{2}L(\bfY, \bfX, t) 
	%	& = &
		=
		\frac{\exp\left(\tilde{\bfX}^{T}t\right)}{\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)^{2}}\cdot\tilde{\bfX}\tilde{\bfX}^{T}$.
	%\end{eqnarray*}
	Under the assumption $\bbE\tilde\bfX\tilde\bfX^{T}<\infty$, the Dominated Convergence Theorem yields:	
	%For all $\bfY$, $\bfX$ and $t\in \bbR^{p+1}$, we have:
	%\begin{eqnarray*}
	%	\left[\left(2\bfY-1\right) - \frac{\exp\left(\tilde{\bfX}^{T}t\right)}{1+\exp\left(\tilde{\bfX}^{T}t\right)}\right]
	%	& \le & 
	%	2, \mbox{ and }
	%	\\
	%	\frac{\exp\left(\tilde{\bfX}^{T}t\right)}{\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)^{2}}
	%	& \le & 1,
	%\end{eqnarray*}
	%so, using the assumptions on the moments of $\bfX$, we know that:
	%\begin{eqnarray*}
	%	\bbE\left[\left|\nabla_{t}L(\bfY, \bfX, t)\right|\right]
	%	& \le &
	%	2\max\left[1, \max_{1\le j\le p}\bbE \left|\bfX_{j}\right|\right] < \infty, \mbox{ and}
	%	\\
	%	\bbE\left[\left|\nabla_{t}^{2}L(\bfY, \bfX, t)\right|\right]
	%	& \le &
	%	\bbE \left[\bfQ(\bfX)\right] < \infty.
	%\end{eqnarray*}
	%Using the Dominated Convergence Theorem we get that:
	\begin{eqnarray*}
		\nabla_{t}R(t) 
		& = & 
		%\bbE\left[\nabla_{t}L(\bfY, \bfX, t)\right] 
		%= 
		%\bbE\left[\left(\bbE\left(\bbI(\bfY=1)|\bfX\right)-\frac{\exp(\tilde{\bfX}^{T}t)}{1+\exp(\tilde{\bfX}^{T}t)}\right)\cdot\tilde{\bfX}\right]
		%\\
		%& = & 
		\bbE\left[\left(p(\bfX)-\frac{\exp(\tilde{\bfX}^{T}t)}{1+\exp(\tilde{\bfX}^{T}t)}\right)\cdot\tilde{\bfX}\right], \mbox{ and }
		\\
		\nabla^{2}_{t}R(t) 
		& = & 
		%\bbE\left[\nabla^{2}_{t}L(\bfY, \bfX, t)\right] 
		%=
		\bbE
		\left[
		\frac
		{\exp\left(\tilde{\bfX}^{T}t\right)}
		{\left(1+\exp\left(\tilde{\bfX}^{T}t\right)\right)^{2}}
		\cdot
		\tilde{\bfX}\tilde{\bfX}^{T}\right].
	\end{eqnarray*}
	We now prove that the Hessian $\nabla^{2}_{t}R(\theta)$ is a strictly positive definite matrix.
	Let $\Psi(\tilde\bfX) = \frac{\exp\left(\tilde{\bfX}^{T}\theta\right)}{\left(1+\exp\left(\tilde{\bfX}^{T}\theta\right)\right)^{2}}$, $\xi = \inf_{\|\bfX\|\le S} \frac{\exp(\alpha+\bfX^{T}\beta)}{\left[1+\exp(\alpha+\bfX^{T}\beta)\vphantom{\int_{0}^{1}}\right]^{2}}>0$, for $\bfM\in\bbR$ write
	\begin{eqnarray*}
	\nabla^{2}_{t}R(\theta)
	& = &
	\bbE
	\left[
	\Psi(\tilde\bfX)
	Q(\bfX)
	\bbI(\|\tilde\bfX\|\le \bfM)
	\right]
	+
	\bbE
	\left[
	\Psi(\tilde\bfX)
	Q(\bfX)
	\bbI(\|\tilde\bfX\|> \bfM)
	\right]
	\\
	& \succeq & 
	\xi	\left[Q(\bfX)\bbI(\|\tilde\bfX\|\le \bfM)\right]
	+
	\bbE
	\left[
	\Psi(\tilde\bfX)
	Q(\bfX)
	\bbI(\|\tilde\bfX\|> \bfM)
	\right]
	.
	\end{eqnarray*}
	Since $\bbE\left[Q(\bfX)\right] = \lim_{s\rightarrow\infty}\bbE\left[Q(\bfX)\cdot\bbI(\|\bfX\|\le s)\right]\succ0$, we can choose $\bfM$ large enough so the first term in the sum is positive definite.
	The proof is complete because the second term in the sum is a positive semi-definite matrix.

\textbf{Proof of L4)}
%	\item [L4)]	
	The loss function corresponds to the neg-loglikelihood function of a canonical exponential family and is thus convex.
	As the risk is an expected value of convex functions, it is also convex.
%\end{enumerate}
\end{proof}	

\begin{proof}[Proof of Lemma \ref{result:variance_and_hessian_for_hinge_loss}]
In the interest of space, we only outline the proof here.
A detailed proof is given in a technical report version of this paper.
Throughout the proof of Lemma \ref{result:variance_and_hessian_for_hinge_loss}, we denote $\tilde{\bfX} = \left[\begin{array}{cc}1 & \bfX^{T}\end{array}\right]^{T}$.
\\
\textbf{Proof of L1)}
	For the hinge loss function, we can prove that
	\begin{eqnarray*}
		\lim_{\|t\|_{2}\rightarrow\infty}
		\bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]
		& = &
		\infty,
	\end{eqnarray*}
	which ensures existence of a minimized. 
	Uniqueness follows from positive definiteness of the Hessian at the minimizer proven below.

	%We first prove that a minimizer exist. 
	%Given that the risk function is continuous, it is enough to prove that for large enough $M$ the closed set $\mcalS(M) = \left\{t\in \bbR^{p}: \bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]\le M\right\}$ is bounded.
	%We establish boundedness of $\mcalS(M)$ by proving that $\mcalS(M)$ is contained on a finite box around the origin.
	%Letting $e_{j}$ be a unit vector with a $1$ in its $j$-th entry and zeroes in all other components, it is sufficient to prove that, for any $M$ and each $j=1, \ldots, p+1$, there exist $\gamma_{j, M}$ such that:
	%\begin{eqnarray}
	%	\label{equation:out_of_box_inclusion}
	%	\left|\langle t, e_{j}\rangle\right| > \gamma_{j, M} & \Rightarrow & \bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]>M.
	%\end{eqnarray}
	%To prove the assertion in $\eqref{equation:out_of_box_inclusion}$, let $t$ be a non-zero vector with $u = \langle t, e_{j}\rangle \neq 0$, so $t$ can be written as $t = u e_{j} + v$, for some $v$ with $\langle v, e_{j}\rangle = 0$.
	%The risk function at $t$ becomes:
	%\begin{eqnarray*}
	%	\bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]
	%	& = &		\bbE\left[\left|1-u\cdot\tilde{\bfX}^{T}e_{j}-\tilde{\bfX}^{T}v\right|\bbI\left(\bfY=1\right)\right]
	%	+		\bbE\left[\left|1+u\cdot\tilde{\bfX}^{T}e_{j}-\tilde{\bfX}^{T}v\right|\bbI\left(\bfY=-1\right)\right]
	%	\\
	%	& \ge &
	%	\bbE\left[\left|u\cdot\tilde{\bfX}^{T}e_{j}+\tilde{\bfX}^{T}v\right|\right]-1
	%	\\
	%	& \ge &
	%	\inf_{v\in \mcalO(e_{j})}
	%	\bbE\left[\left|u\cdot\tilde{\bfX}^{T}e_{j}+\tilde{\bfX}^{T}v\right|\right]-1
	%	\\
	%	& = &
	%	|u|\cdot
	%	\inf_{v\in \mcalO(e_{j})}
	%	\bbE\left[\left|\tilde{\bfX}^{T}e_{j}+\tilde{\bfX}^{T}v\right|\right]-1,
	%\end{eqnarray*}
	%where $\mcalO(e_{j})$ is the set of all vectors orthogonal to $e_{j}$. Because $e_{j}$ has unit norm, $\|e_{j}+v\|\ge 1$ for all $v\in \mcalO(e_{j})$ and it follows that $\{e_{j}+v:v\in\mcalO(e_{j}) \}\subset \{v:\|v\|\ge 1\}$, yielding:
	%\begin{eqnarray*}
	%	\bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]
	%	& \ge &
	%	|u|\cdot
	%	\inf_{v:\|v\|\ge 1}
	%	\bbE\left[\left|\tilde{\bfX}^{T}v\right|\right]-1
	%	=
	%	|u|\cdot
	%	\inf_{v:\|v\| = 1}
	%	\bbE\left[\left|\tilde{\bfX}^{T}v\right|\right]-1,
	%\end{eqnarray*}
	%where the equality follows from noticing that $\left|\tilde{\bfX}^{T}v\right|$ is increasing in $\left|v\right|$.
	%If we can find $c>0$, such that  $\inf_{v:\|v\|= 1}\bbE\left[\left|\tilde{\bfX}^{T}v\right|\right]>c$, it is possible to find the $\gamma_{j,M}$ we want.
	%To find such a positive lower bound,  define the compact set $\bfK = \{\tilde{x}\in \bbR^{p+1}:\|\tilde{x}\|_{2}\le\bfC\}$ for some constant $\bfC$.
	%Since it is assumed that $f_{\bfX}(\bfx)>0$ is continuous for all $\bfx\in\bbR^{p}$, we get that $f^{*}=\min_{\bfx\in \bfK}>0$.
	%Now, letting $\mu(\bfA)$ denote the Lebesgue measure of a set $\bfA\subset\bbR^{p+1}$, we have:
	%\begin{eqnarray*}
	%	\inf_{v:\|v\|= 1}
	%	\bbE\left[\left|\tilde{\bfX}^{T}v\right|\right]
	%	& \ge &
	%	\eta
	%	\cdot
	%	\inf_{v:\|v\|\ge 1}
	%	\bbP\left[\left|\tilde{\bfX}^{T}v\right|>\eta\right]
	%	\\
	%	& \ge &
	%	\inf_{v:\|v\|\ge 1}
	%	\bbP\left[\tilde{\bfX}^{T}v>\eta, \mbox{ and } \tilde{\bfX}\in \bfK \right]
	%	\\
	%	& \ge &
	%	f^{*}
	%	\cdot
	%	\inf_{v:\|v\|\ge 1}
	%	\mu\left(\{\bfx:\tilde{\bfx}^{T}v>\eta\}\right).
	%	\\
	%	& = &
	%	f^{*}
	%	\cdot
	%	\mu\left(\{\bfx:\tilde{\bfx}^{T}e_{1}>\eta\}\right)=:c_{\eta}>0,
	%\end{eqnarray*}
	%where the last equality follows from noticing that, because of symmetry:
	%\begin{eqnarray*}
	%	\mu\left(\{\bfx:\tilde{\bfx}^{T}v>\eta\}\right) 
	%	= 
	%	\mu\left(\{\bfx:\tilde{\bfx}^{T}e_{1}>\eta\}\right), \mbox{ for all }v\in \bbR^{p+1}: \|v\|_{2}=1.
	%\end{eqnarray*}
	%
	%Using the strictly positive lower bound afforded by $c_{\eta}$, we get:
	%\begin{eqnarray*}
	%	|u| = \left|\langle t, e_{j}\rangle\right| > \gamma_{j, M}:= \frac{M+1}{f^{*}c_{\eta}} , \mbox{ for some } j=1, \ldots, p 
	%	&\Rightarrow& 
	%	\bbE\left[\left|1-\bfY\tilde{\bfX}^{T}t\right|_{+}\right]>M.
	%\end{eqnarray*}
	%
	%Uniqueness of the minimizer follows from strict convexity of the risk function under the assumptions made.
	%Strict convexity of the risk function in its turn is proved below, by showing the Hessian matrix for the risk is everywhere strictly positive definite.
	
	%\item [L2)] 
	\textbf{Proof of L2)}
	For all $t\in \bbR^{p+1}$:
	\begin{eqnarray*}
		\bbE\left[\left|L(\bfZ, t)\right|\right]
		\le
		\bbE\left[\max\left\{\left|1-\tilde{\bfX}t\right|, \left|1+\tilde{\bfX}t\right|\right\}\right]
		%\le
		%1+\bbE\left[\left|\tilde{\bfX}t\right|\right]
		\le
		1+\sqrt{t^{t}\cdot\bbE\left[\tilde{\bfX}^{T}\tilde{\bfX}\right]\cdot t},
	\end{eqnarray*}
	which is bounded given the assumptions on the distribution of $\bfX$.
	
	%\item [L3)]
	\textbf{Proof of L3)}
	
		The hinge loss is not differentiable on the set $\{\bfX: \tilde{\bfX}t=1 \mbox{ or } \tilde{\bfX}t=-1\}$, which under the assumed conditions has zero probability.
		At all other points, hinge loss function has derivative with respect to $t$
		\begin{eqnarray*}
			\nabla_{t}L(\bfZ, t)
			& = & 
			\tilde{\bfX}
			\cdot
			\left[
			\bbI(\bfY=1)\cdot\bbI(\tilde{\bfX}t-1<0)
			-
			\bbI(\bfY=-1)\cdot\bbI(\tilde{\bfX}t+1>0)
			\right]
		\end{eqnarray*}
		
		To obtain the Hessian, write the SVM risk as $R(t) = R_{1}(t) + R_{2}(t)$, with
		\begin{eqnarray*}
		R_{1}\left(t\right)	& := & \bbE
		                               \left[
		                               p\left(\bfX\right)
		                               \cdot
			                           \left(1-\tilde{\bfX}t\right)
		                               \cdot
		                               \bbI\left(1-\tilde{\bfX}t>0\right)
		                               \right],\mbox{ and }
		\\
		R_{2}\left(t\right)	& := & \bbE
		                               \left[
								      \left(1-p\left(\bfX\right)\right)
								      \cdot
								      \left(\tilde{\bfX}t-1\right)
								      \cdot
								      \bbI\left(\tilde{\bfX}t-1>0\right)
		                               \right].
		\end{eqnarray*}
		Let
			$
			\nabla_{t}R_{1}(t) 
			:= 
			\bbE\left[
			p(\tilde{\bfX})
			\cdot 
			\bbI\left(1-\tilde{\bfX}t>0\right) 
			\cdot 
			\tilde{\bfX}
			\right]
			$ 
			and 
			$
			\nabla^{2}_{t}R_{1}(t) 
			:=
			\bbE\left[
			p(\tilde{\bfX})
			\cdot
			\delta(1-\tilde{\bfX}t) 
			\cdot 
			\tilde{\bfX}^{T}
			\tilde{\bfX}
			\right].
			$
		We first show that $r_{1}(t) := R_{1}(t+\Delta t) - R_{1}(t) = \nabla_{t}R_{1}(t)\cdot\Delta t = o(\|\Delta t\|)$. 
		To do that, let $\bfd_{k}=\frac{\Delta t_{k}}{|\Delta t_{k}|}$ and write
		\begin{small}
		\begin{eqnarray*}
		\frac{R_{1}(t+\Delta t_{k}) - R_{1}(t)}{\Delta t_{k}}
		& = &
		\bbE
		\left[
		\frac
		{
		p(\tilde{\bfX})
		\left(1-\tilde{\bfX}t\right)
		\left[
		  \bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		  - 
		  \bbI\left(1-\tilde{\bfX}t>0\right) 
		\right]
		}{\tilde{\bfX}\Delta t}
		\cdot
		\tilde{\bfX}
		\right]
		\bfd_{k}
		\\
		& &
		-
		\bbE
		\left[
		p(\tilde{\bfX})
		\cdot 
		\bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		\cdot 
		\tilde{\bfX}
		\right]
		\bfd_{k}.
		\end{eqnarray*}
		\end{small}
		Using the Dominated Convergence Theorem to take the limit as $\Delta t\downarrow 0$ and collecting the limit of the multiplier of $\bfd_{k}$ yields
		\begin{small}
		\begin{eqnarray*}
		\nabla_{t}R_{1}(t)
		& = &
		\lim_{|\Delta t|\rightarrow 0}
		\bbE
		\left[
		\frac
		{
		p(\tilde{\bfX})
		\left(1-\tilde{\bfX}t\right)
		\left[
		  \bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		  - 
		  \bbI\left(1-\tilde{\bfX}t>0\right) 
		\right]
		}{\tilde{\bfX}\Delta t}
		\cdot
		\tilde{\bfX}
		\right]
		\\
		& &
		-
		\lim_{|\Delta t|\rightarrow 0}
		\bbE
		\left[
		p(\tilde{\bfX})
		\cdot 
		\bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		\cdot 
		\tilde{\bfX}
		\right]
		\\
		& = &
		\bbE
		\left[
		p(\tilde{\bfX})
		\left(1-\tilde{\bfX}t\right)
		\delta(1-\tilde{\bfX}^{T}t)
		\cdot
		\tilde{\bfX}
		\right]
		-
		\bbE
		\left[
		p(\tilde{\bfX})
		\cdot 
		\bbI\left(1-\tilde{\bfX}t>0\right) 
		\cdot 
		\tilde{\bfX}
		\right]
		\\
		& = & 
		-
		\bbE
		\left[
		p(\tilde{\bfX})
		\cdot 
		\bbI\left(1-\tilde{\bfX}t>0\right) 
		\cdot 
		\tilde{\bfX}
		\right].
		\end{eqnarray*}
		\end{small}
		
		To obtain the second differential for $R_{1}(t)$, write the residuals from the approximation from the first differential:
		\begin{small}
		\begin{eqnarray*}
		\frac
		{
		r_{1}(\Delta t)
		}
		{|\Delta t_{k}|^{2}}
		%&:=&
		%\frac
		%{
		%R_{1}(t+\Delta t_{k})-R_{1}(t)-\nabla_{t}R_{1}(t)^{T}\cdot\Delta t_{k}
		%}
		%{|\Delta t_{k}|^{2}}
		%\\
		& = &
		\bfd_{k}
		\bbE
		\left[
		\frac{
		p(\tilde{\bfX})
		\cdot 
		\tilde{\bfX}^{T}
		\cdot
		\left[
		  \bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		  - 
		  \bbI\left(1-\tilde{\bfX}t>0\right) 
		\right]
		\cdot 
		\left(1-\tilde{\bfX}t\right)
		\cdot 
		\tilde{\bfX}
		}
		{\Delta t^{T}\tilde{\bfX}\tilde{\bfX}^{T}\Delta t}
		\right]
		\bfd_{k}
		\\
		& &
		-
		\bfd_{k}
		\cdot
		\bbE
		\left[
		\frac{
		p(\tilde{\bfX})
		\cdot 
		\tilde{\bfX}^{T}
		\cdot
		\left[
		\bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t\right) 
		-
		\bbI\left(1-\tilde{\bfX}t>0\right) 
		\right]
		\cdot 
		\tilde{\bfX}
		}
		{\tilde{\bfX}\Delta t}
		\right]
		\cdot
		\bfd_{k}
		\end{eqnarray*}
		\end{small}
	The second derivative is obtained using the Dominated Convergence Theorem to compute the limits of the terms in the sum.
	For the second term, the limit follows directly from pointwise convergence to a Dirac delta function:
	\begin{small}
	\begin{eqnarray*}
	\begin{array}{ccl}
	\lim\limits_{|\Delta t|\rightarrow 0}
	\bbE
	\left[
	\frac{
	p(\tilde{\bfX})
	\cdot 
	\tilde{\bfX}
	\cdot
	\left[
	\bbI\left(1-\tilde{\bfX}^{T}t>\tilde{\bfX}^{T}\Delta t\right) 
	-
	\bbI\left(1-\tilde{\bfX}^{T}t>0\right) 
	\right]
	\cdot 
	\tilde{\bfX}^{T}
	}
	{\tilde{\bfX}^{T}\Delta t}
	\right]
	=
	-
	\bbE
	\left[
	p(\tilde{\bfX})
	\cdot
	\delta(1-\tilde{\bfX}^{T}t) 
	\cdot
	\tilde{\bfX}
	\tilde{\bfX}^{T}
	\right].
	&&
	\end{array}
	\end{eqnarray*}
	\end{small}
	
	To obtain the limit for the other term, let $W = R\tilde{\bfx} = \left[\begin{array}{cc}\bfw_{1} & \bfw_{2}\end{array}\right] \in \bbR\times \bbR^{p-1}$ be a linear rotation of $\tilde{x}$ such that $\bfw_{1} = \tilde{\bfx}^{T}t$, and let $F_{\tilde{\bfx}}$, $F_{\bfw_{2}}$, and  $f_{\bfw_{1}|\bfw_{2}}$ denote the distributions of $\tilde{X}$, $W_{2}$ and the conditional distribution of $W_{1}$ given $W_{2}$ respectively.
	Then write
	\begin{small}
	\begin{eqnarray*}
	\begin{array}{lc}
%	\lim_{|\Delta t_{k}|\rightarrow 0}
	\bbE
	\left[
	\frac{
	p(\tilde{\bfX})
	\cdot 
	\tilde{\bfX}^{T}
	\cdot
	\left[
	  \bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t_{k}\right) 
	  - 
	  \bbI\left(1-\tilde{\bfX}t>0\right) 
	\right]
	\cdot 
	\left(1-\tilde{\bfX}t\right)
	\cdot 
	\tilde{\bfX}
	}
	{\Delta t_{k}^{T}\tilde{\bfX}\tilde{\bfX}^{T}\Delta t_{k}}
	\right]
	& 
	= 
	\\
%	\lim_{|\Delta t_{k}|\rightarrow 0}
	\int
	\left[
	\frac{
	\left(1-\tilde{\bfx}t\right)
	\cdot
	\left[
	\bbI\left(1-\tilde{\bfx}t>\tilde{\bfx}\Delta t_{k}\right) 
	- 
	\bbI\left(1-\tilde{\bfx}t>0\right) 
	\right]
	}
	{\Delta t_{k}^{{T}}\tilde{\bfx}^{T}\tilde{\bfx}^{T}\Delta t_{k}}
	\cdot	
	p(\tilde{\bfx})
	\cdot	
	\tilde{\bfx}
	\tilde{\bfx}^{T}
	\right]
	\mbox{d}F_{\tilde{\bfx}}\left(\tilde{\bfx}\right)
	& 
	= 
	\\
%	\lim_{|\Delta t_{k}|\rightarrow 0}
	\int
	\int
	\frac{
	\left(1-\bfw_{1}\right)
	\cdot
	\left[
	\bbI\left(1-\bfw_{1}>\tilde{\bfx}(\bfw)\Delta t_{k}\right) 
	- 
	\bbI\left(1-\bfw_{1}>0\right) 
	\right]
	}
	{\Delta t_{k}^{T}\tilde{\bfx}(\bfw)\tilde{\bfx}^{T}(\bfw)\Delta t_{k}}
	s(\bfw_{1}, \bfw_{2})
	dF_{\bfw_{1}|\bfw_{2}}(\bfw_{1}\left|\bfw_{2}\right.)
	dF_{\bfw_{2}}(\bfw_{2}),
	&
%	& = & 
%	\\
%	-
%	\frac{1}{2}
%	\bbE
%	\left[
%	p(\tilde{\bfX})
%	\cdot
%	\delta(1-\tilde{\bfX}^{T}t) 
%	\cdot
%	\tilde{\bfX}
%	\tilde{\bfX}^{T}
%	\right].
%	&&
	\end{array}
	\end{eqnarray*}
	\end{small}
	where we used the notation $s(\bfw_{1}, \bfw_{2}) := p(\tilde\bfx(\bfw_{1}, \bfw_{2}))\bfx(\bfw_{1}, \bfw_{2})\bfx(\bfw_{1}, \bfw_{2})^{T}$.

	To obtain the limit, write the inner integral as:
	\begin{small}
	\begin{eqnarray*}
		\begin{array}{ll}
		\int
		\left[
		\frac{
		\left(1-\bfw_{1}\right)
		\cdot
		\left[
		\bbI\left(1-\bfw_{1}>\tilde{\bfx}(\bfw_{1}, \bfw_{2})\Delta t_{k}\right) 
		- 
		\bbI\left(1-\bfw_{1}>0\right) 
		\right]
		}
		{\Delta t_{k}^{T}\tilde{\bfx}(\bfw_{1}, \bfw_{2})\tilde{\bfx}^{T}(\bfw)\Delta t_{k}}
		\cdot	
%		p(\tilde{\bfx}(\bfw_{1}, \bfw_{2}))
%		\cdot	
%		\tilde{\bfx}(\bfw_{1}, \bfw_{2})
%		\tilde{\bfx}^{T}(\bfw_{1}, \bfw_{2})
		s(\bfw_{1}, \bfw_{2})
		\right]
		dF_{\bfw_{1}|\bfw_{2}}(\bfw_{1}\left|\bfw_{2}\right)
		&
		=
		\\
		\int
		\left[
		\frac{
		v
		\cdot
		\left[
		\bbI\left(v>\tilde{\bfx}(\bfw_{1}, \bfw_{2})\Delta t_{k}\right) 
		- 
		\bbI\left(v>0\right) 
		\right]
		}
		{\Delta t_{k}^{T}\tilde{\bfx}(1-v, \bfw_{2})\tilde{\bfx}^{T}(\bfw)\Delta t_{k}}
		\cdot	
%		p(\tilde{\bfx}(1-v,\bfw_{2}))
%		\cdot	
%		\tilde{\bfx}(1-v, \bfw_{2})
%		\tilde{\bfx}^{T}(1-v, \bfw_{2})
		s(1-v, \bfw_{2})
		\right]
		dF_{\bfw_{1}|\bfw_{2}}(1-v\left|\bfw_{2}\right)
		&
		=
		\\
		-
		\int
		\left[
		\frac{1}{2}
		\cdot	
%		p(\tilde{\bfx}(1-v,\bfw_{2}))
%		\cdot	
%		\tilde{\bfx}(1-v, \bfw_{2})
%		\tilde{\bfx}^{T}(1-v, \bfw_{2})
		s(\bfw_{1}, \bfw_{2})
		\cdot
		\delta(1-\bfw_{1})
		\right]
		dF_{\bfw_{1}|\bfw_{2}}(\bfw_{1}\left|\bfw_{2}\right)
		+
		o(\|\Delta t\|).
		\end{array}
	\end{eqnarray*}
	\end{small}
	Plugging that back into the expression for the expected value, we get:
	\begin{small}
	\begin{eqnarray*}
		\begin{array}{ll}
		\lim_{|\Delta t_{k}|\rightarrow 0}
		\bbE
		\left[
		\frac{
		p(\tilde{\bfX})
		\cdot 
		\tilde{\bfX}^{T}
		\cdot
		\left[
		  \bbI\left(1-\tilde{\bfX}t>\tilde{\bfX}\Delta t_{k}\right) 
		  - 
		  \bbI\left(1-\tilde{\bfX}t>0\right) 
		\right]
		\cdot 
		\left(1-\tilde{\bfX}t\right)
		\cdot 
		\tilde{\bfX}
		}
		{\Delta t_{k}^{T}\tilde{\bfX}\tilde{\bfX}^{T}\Delta t_{k}}
		\right]
		& = 
		\\
		-
		\int
		\left[
		\int
		\left[
		\frac{1}{2}
		\cdot	
%		p(\tilde{\bfx}(1-v,\bfw_{2}))
%		\cdot	
%		\tilde{\bfx}(1-v, \bfw_{2})
%		\tilde{\bfx}^{T}(1-v, \bfw_{2})
		s(\bfw_{1}, \bfw_{2})
		\cdot
		\delta(1-\bfw_{1})
		\right]
		dF_{\bfw_{1}|\bfw_{2}}(\bfw_{1}\left|\bfw_{2}\right)
		\right]
		dF{\bfw_{2}}(\bfw_{2})
		& = 
		\\
		-\frac{1}{2}
		\cdot
		\bbE
		\left[
		p(\tilde{\bfX})
		\cdot 
		\tilde{\bfX}
		\tilde{\bfX}^{T}
		\cdot
		\delta(1-\tilde{\bfX}^{T}t)
		\right].
		&
	\end{array}
	\end{eqnarray*}
	\end{small}
	
	Summing the two terms (and taking into account the factor $\frac{1}{2}$ in the Taylor expansion) yield $\nabla_{t}^{2}R_{1}(t) = 
	\bbE
	\left[
	p(\tilde{\bfX})
	\cdot
	\delta(1-\tilde{\bfX}^{T}t) 
	\cdot
	\tilde{\bfX}
	\tilde{\bfX}^{T}
	\right]$.
	For $R_{2}$, analogous steps yield $\nabla_{t}R_{2}(t)
		=
		\bbE
		\left[
		\left(1-p(\tilde{\bfX})\right)
		\cdot 
		\bbI\left(1+\tilde{\bfX}t>0\right) 
		\cdot 
		\tilde{\bfX}
		\right]$ and 
		$\nabla_{t}^{2}R_{2}(t)
		 =  
		\bbE
		\left[
		\left(1-p(\tilde{\bfX})\right)
		\cdot
		\delta(1+\tilde{\bfX}^{T}t) 
		\cdot
		\tilde{\bfX}
		\tilde{\bfX}^{T}
		\right]$.
		The result follows from summing the differentials for $R_{1}(t)$ and $R_{2}(t)$.
	
	Finally, we prove that the minimizer of the SVM risk is unique by establishing that $\nabla_{t}^{2}R(\theta)$ is strictly positive definite.
	To do that, first write:
	\begin{eqnarray*}
	\nabla_{t}^{2}R(t)
	& = & 
	\bbE
	\left[
	Q(\bfX)
	\left|
	\alpha+\bfX^{T}\beta = 1
	\right.
	\right]
	\cdot 
	\bbP\left(\bfY=1\left|\alpha+\bfX^{T}\beta=1\right.\right)
	\cdot 
	\tilde{f}(1)
	\\
	&&
	+
	\bbE
	\left[
	Q(\bfX)
	\left|
	\alpha+\bfX^{T}\beta = -1
	\right.
	\right]
	\cdot 
	\bbP\left(\bfY=-1\left|\alpha+\bfX^{T}\beta=1\right.\right)
	\cdot 
	\tilde{f}(-1),
	\end{eqnarray*}
	where $\tilde{f}$ denote the density of the random variable $\alpha+\bfX^{T}\beta$.
	Given assumption C2, $\tilde{f}(-1)>0$ and $\tilde{f}(1)>0$.
	In addition, assumption C3 gives that $\bbP\left(\bfY=-1\left|\alpha+\bfX^{T}\beta=1\right.\right)>0$ and $\bbP\left(\bfY=1\left|\alpha+\bfX^{T}\beta=1\right.\right)>0$.
	It is thus, enough to prove that either $\bbE\left[Q(\bfX)\left|\alpha+\bfX^{T}\beta = -1\right.\right]$ or $\bbE\left[Q(\bfX)\left|\alpha+\bfX^{T}\beta = -1\right.\right]$ is strictly positive definite (or both).
	
	Define $\bfv_{\beta} = \frac{\beta}{\|\beta\|}$, the unit vector in the direction of $\beta$.
	The condition $\alpha+\bfX^{T}\beta = \kappa$ is equivalent to $\bfX^{T}\bfv_{\beta} = \frac{\kappa-\alpha}{\|\beta\|}$, so for any scalar $\kappa$:
	\begin{eqnarray*}
		\bbE\left[Q(\bfX)\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]
		& = &
		\bbE\left[Q(\bfX)\left|\bfX^{T}\bfv_{\beta} = \frac{\kappa-\alpha}{\|\beta\|}\right.\right].
	\end{eqnarray*}
%	Now, defining $D(\kappa):=\bbE\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]$, we know that:
%	\begin{eqnarray*}
%		\bbE\left[Q(\bfX)\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]
%		& = &
%		\left[
%		\begin{array}{cc}
%			1 
%			& 
%			D(\kappa)
%			%\bbE\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]^{T}
%			\\
%			%\bbE\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]
%			D(\kappa)
%			& 
%			%\bbE\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]
%			%\bbE\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]^{T}
%			D(\kappa)D(\kappa)^{T}
%		\end{array}
%		\right]
%		\\
%		& &
%		+
%		\left[
%		\begin{array}{cc}
%			0 
%			& 
%			\bfzero^{T}
%			\\
%			\bfzero
%			& 
%			\var\left[\bfX\left|\alpha+\bfX^{T}\beta = \kappa\right.\right]
%		\end{array}
%		\right].
%	\end{eqnarray*}
%	Decompose $\bfX$ into a projection on the direction $\bfv_{\beta}$ and a residual that belongs in the orthogonal complement of the space spanned by $\bfv_{\beta}$:
%	$\bfX = \bfv_{\beta}\left(\bfv_{\beta}^{T}\bfX\right) + \left[\bfI_{p}-\bfv_{\beta}\bfv_{\beta}^{T}\right]\bfX$.
%	Because $\var(\bfX)$
	Then notice that:
	\begin{eqnarray*}
		\bbE\left[Q(\bfX)\left|\bfX^{T}\bfv_{\beta}=\frac{\kappa-\alpha}{\|\beta\|}\right.\right]
		\succeq
		\left[
		\begin{array}{cc}
		1
		&
		\left(\frac{\kappa-\alpha}{\|\beta\|}\right)\bfv_{\beta}^{T}
		\\
		\left(\frac{\kappa-\alpha}{\|\beta\|}\right)\bfv_{\beta}
		&
		\left(\frac{\kappa-\alpha}{\|\beta\|}\right)^{2}\left(\bfv_{\beta}\bfv_{\beta}^{T}\right)
		+
		\var\left(\bfX\left|\bfX^{T}\bfv_{\beta}=\frac{\kappa-\alpha}{\|\beta\|}\right.\right)			
		\end{array}
		\right],
	\end{eqnarray*}
	where $A\succeq B$ denotes that $A-B$ is positive semi definite.
	Because $\bbE\bfX\bfX^{T}$ is assumed to be non-singular, $\var\left(\bfX\left|\bfX^{T}\bfv_{\beta}=\frac{\kappa-\alpha}{\|\beta\|}\right.\right)$ has rank $p-1$ and $\var\left(\bfX\left|\bfX^{T}\bfv_{\beta}=\frac{\kappa-\alpha}{\|\beta\|}\right.\right)\bfv_{\beta}=0$.
	Thus, as long as $\kappa\neq \alpha$, $\bbE\left[Q(\bfX)\left|\bfX^{T}\bfv_{\beta} = \frac{\kappa-\alpha}{\|\beta\|}\right.\right]$ is stricly positive definite.
	
	If $\alpha\not\in\{-1,1\}$, both terms in the sum defining $\nabla_{t}^{2}R(\theta)$ are strictly positive definite.
	If $\alpha\in\{-1,1\}$, one of the terms in the sum defining $\nabla_{t}^{2}R(\theta)$ is singular, but the other is necessarily strictly positive definite.
	Thus, it follows that $\nabla_{t}^{2}R(\theta)$ is strictly positive definite as stated.`'
	
	
	%\item [L4)] 
	
	\textbf{Proof of L4)}
	We can write $\|1-\tilde{\bfX}t\|_{+}$ as the maximum between the constant function $0$ and the function $\bfY-\tilde{\bfX}t$ which is linear -- thus, convex -- on $t$. Since it is the maximum between two convex functions on $t$, $\|\bfY-\tilde{\bfX}t\|_{+}$ is convex on $t$. A similar argument yields that $\|\tilde{\bfX}t-1\|_{-}$ is convex on $t$.
	
	The loss function $L(\bfZ, t)$ is written as the sum (with positive weights) of convex functions, which proves that AL.IV holds for the SVM loss function.

%\end{enumerate}

\end{proof}	


